Forward Link Analysis for Full-Duplex Cellular Networks with Low Resolution ADC/DAC

In this work, we consider a full-duplex (FD) massive multiple-input multiple-output (MIMO) cellular network with low resolution analog-to-digital converters (ADCs) and digital-to-analog converters (DACs). Our first contribution is to propose a unified framework for forward link analysis where matched filter precoders are applied at the FD base stations (BSs) under channel hardening. Second, we derive expressions for the signal-to-quantization-plus-interference-plus-noise ratio (SQINR) for general and special cases. Finally, we quantify effects of quantization error, pilot contamination, and full duplexing for a hexagonal cell lattice on spectral efficiency and cumulative distribution function (CDF) to show that FD outperforms half duplex (HD) in a wide variety of scenarios.

==> asymptotic.tex <==
\section{Asymptotic Analysis and Power Scaling Laws}
In the section, we investigate the effects of the number of quantization bits, the number of antennas at the BS, the number of users, the power budgets of the BS and each user on the spectral efficiency performance for forward link.

\begin{lemma}\label{lemma2}
For a fixed power budget, fixed number of transmit antennas and full-resolution ($b \rightarrow \infty$, $ \alpha = 1$), the spectral efficiency converges to (\ref{downlinklemma2}).
\end{lemma}
In (\ref{downlinklemma2}), the quantization error introduced by the finite-resolution ADC/DAC is eliminated for infinite resolution. When the number of antennas is held fixed, the average forward link spectral efficiency becomes constant. Though increasing the ADC/DAC resolution can improve the performance, the spectral efficiency is limited.
\begin{figure*}
\begin{equation}\label{downlinklemma2}
\begin{split}
&\frac{\bar{\mathcal{I}}^\mathsf{MF}}{B} \rightarrow\\& \log\left( 1 + \frac{ \frac{N_{\mathsf{a}}}{\varrho + \frac{P_k^u}{P_u} \mathsf{SNR}_k^d + \sum_{\ell \in \mathcal{C}} \frac{P_{\ell,k}^u}{P_u}\mathsf{SNR}_{\ell,k}^d  } \frac{P_{k}^u}{P_u} \frac{P_k^d}{P_d} \left(\mathsf{SNR}^d_k\right)^2}  {1+ \sum_\ell \mathsf{SNR}_{\ell,k}^d + \sum_{\ell \in \mathcal{C}}  \frac{  N_{\mathsf{a}}}{\varrho+\frac{P_k^u}{P_u}\mathsf{SNR}_{\ell,k}^d + \sum_{l\in \mathcal{C}}\frac{P_{l,k}^u}{P_u}\textsf{SNR}_{\ell,(l,k)}^d}\frac{P_{k}^u}{P_u}\frac{P_{\ell,k}^d}{P_d}\left(\mathsf{SNR}_{\ell,k}^d\right)^2 +  \sum_{\ell}\sum_{\text{k}=0}^{K_\ell^u-1}\frac{P_{\ell,\text{k}}^u}{P_u}  \mathsf{SNR}_{(\ell,\text{k}),k}^{\text{iui}}  }    \right)
\end{split}
\end{equation}
\end{figure*}

\begin{lemma}\label{lemma3}
For a fixed number of antennas, fixed $b$ and assuming uniform power allocation for forward link, when $\mathsf{SNR}_k^d \rightarrow \infty$, the spectral efficiency converges to 
\end{lemma}
\begin{equation}\label{downlinklemma3}
\frac{\bar{\mathcal{I}}^\mathsf{MF}}{B} \rightarrow \log\left( 1 + \frac{\alpha N_{\mathsf{a}}}{K^d -\alpha+1} \right)
\end{equation}
In (\ref{downlinklemma3}), the spectral efficiency depends on the number of antennas, quantization bits $b$ and the number of users per cell when the BS transmit power goes infinity. We further observe that the inter-user interference, pilot contamination and the intra-cell/inter-cell interferences are eliminated.
\begin{lemma}\label{lemma4}
If the transmit powers of the BS and each user is scaled with the number of antennas $N_{\mathsf{a}}$ i.e., $P = \frac{E}{N_{\mathsf{a}}}$ where $E$ is fixed, as $N_{\mathsf{a}} \rightarrow \infty$, the spectral efficiency converges to (\ref{downlinklemma4}).
\end{lemma}
\begin{equation}\label{downlinklemma4}
\frac{\bar{\mathcal{I}}^\mathsf{MF}}{B} \rightarrow \log\left(1 + \frac{\alpha^2}{\varrho}\frac{E_k^u}{E_u}\frac{E_k^d}{E_d}\left( \mathsf{SNR}_k^d \right)^2  \right)    
\end{equation}
(\ref{downlinklemma4}) implies that using a proper power scaling and more antennas can wipe out the inter-user interference, the pilot contamination and the inter-cell/intra-cell interferences. The number of quantization bits determines the approximate spectral efficiency when the number of antennas at the BS goes to infinity.
\begin{lemma}\label{lemma5}
If the transmit power and the number of users per cell are fixed, as $N_{\mathsf{a}}/K\rightarrow \infty$, the spectral efficiency converges to (\ref{downlinklemma5}).
\end{lemma}
\begin{figure*}
\begin{equation}\label{downlinklemma5}
 \frac{\bar{\mathcal{I}}^\mathsf{MF}}{B} \rightarrow \log\left(1 + \frac{  \frac{1}{\varrho + \frac{P_k^u}{P_u} \mathsf{SNR}_k^d + \sum_{\ell \in \mathcal{C}} \frac{P_{\ell,k}^u}{P_u}\mathsf{SNR}_{\ell,k}^d  } \frac{P_{k}^u}{P_u} \frac{P_k^d}{P_d} \left(\mathsf{SNR}^d_k\right)^2     }{ \sum_{\ell \in \mathcal{C}}  \frac{  1}{\varrho+\frac{P_k^u}{P_u}\mathsf{SNR}_{\ell,k}^d + \sum_{l\in \mathcal{C}}\frac{P_{l,k}^u}{P_u}\textsf{SNR}_{\ell,(l,k)}^d}\frac{P_{k}^u}{P_u}\frac{P_{\ell,k}^d}{P_d}\left(\mathsf{SNR}_{\ell,k}^d\right)^2 }  \right)
\end{equation}
\end{figure*}
In the absence of pilot contamination, the motivation behind increasing the ratio $N_{\mathsf{a}}/K_\ell$ is that the beam through which each user's signal is received becomes progressively narrower and the interference is naturally rejected. In the presence of the pilot contamination, however, (\ref{downlinklemma4}) corroborates that the SQINR is interference-limited and that the pilot contamination imposes a limit on the SQINR. Eventually, the pilot contamination comes to dominate over the inter-user, intra-cell and inter-cell interference. Heuristic techniques have been proposed to mitigate the pilot contamination such as subspace methods, coordinated pilot assignment, reception and precoding with other-cell awareness and large-scale multicell processing, etc.




